Cross-lingual Transfer of Reward Models in Multilingual Alignment

Reinforcement learning with human feedback (RLHF) is shown to largely benefit from precise reward models (RMs). However, recent studies in reward modeling schemes are skewed towards English, limiting the applicability of RLHF in multilingual alignments. In this work, we investigate the cross-lingual transfer of RMs trained in diverse languages, primarily from English. Our experimental results demonstrate the strong cross-lingual transfer of English RMs, exceeding target language RMs by 3~4% average increase in Multilingual RewardBench. Furthermore, we analyze the cross-lingual transfer of RMs through the representation shifts. Finally, we perform multilingual alignment to exemplify how cross-lingual transfer in RM propagates to enhanced multilingual instruction-following capability, along with extensive analyses on off-the-shelf RMs. We release the code, model, and data.

==> tables/main_table_compressed.tex <==

\begin{table*}[t!]
\centering
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|ccc|ccc|ccc|ccc@{}}
\toprule
 &
  \multicolumn{3}{c|}{\textbf{\textsc{Chinese}}} &
  \multicolumn{3}{c|}{\textbf{\textsc{Italian}}} &
  \multicolumn{3}{c|}{\textbf{\textsc{Spanish}}} &
  \multicolumn{3}{c}{\textbf{\textsc{Korean}}} \\
 &
  \textbf{Target} &
  \textbf{Eng.} &
  $\Delta$  (\%)&
  \textbf{Target} &
  \textbf{Eng.} &
  $\Delta$  (\%)&
  \textbf{Target} &
  \textbf{Eng.} &
  $\Delta$  (\%)&
  \textbf{Target} &
  \textbf{Eng.} &
  $\Delta$  (\%) \\ \midrule
\textbf{Llama-3.2-3B} &65.6  &70.2  & \textbf{\textcolor{red!60}{+7.0}} &73.0  &79.0  & \textbf{\textcolor{red!90}{+8.2}}  &75.0  &79.3  & \textbf{\textcolor{red!45}{+5.7}} &67.3  &71.6  & \textbf{\textcolor{red!80}{+6.4}} \\
\textbf{Qwen2.5-3B}   &69.4  &72.2  &  \textbf{\textcolor{red!50}{+4.0}}  &75.8  &79.0  &  \textbf{\textcolor{red!40}{+4.2}}  &75.5  &78.1  & \textbf{\textcolor{red!40}{+3.4}} &68.5  &72.8  &  \textbf{\textcolor{red!70}{+6.3}} \\
% \textbf{Phi3-mini} & 63.55 & 69.65 & \textbf{\textcolor{red!85}{+9.60}}  & 72.96 & 74.30 & \textbf{\textcolor{red!20}{+1.84}}  & 71.56 & 73.37 & \textbf{\textcolor{red!25}{+2.53}} & 61.57 & 67.60 & \textbf{\textcolor{red!85}{+9.79}} \\
% \textbf{Gemma2}    & 61.37 & 70.69 & \textbf{\textcolor{red!100}{+15.19}} & 68.54 & 75.91 & \textbf{\textcolor{red!95}{+10.75}} & 68.54 & 73.30 & \textbf{\textcolor{red!60}{+6.94}} & 63.65 & 69.85 & \textbf{\textcolor{red!85}{+9.74}} \\ 
\bottomrule
\end{tabular}%
}
\end{center}
\caption{Multilingual \texttt{RewardBench} evaluation results when trained with the target language ("Target") and English ("Eng.") preference datasets. "$\Delta$" denotes the accuracy gain of reward models trained with the English preference dataset compared to the ones trained with the target language by percentage.}
\label{tab:main_comp}
\end{table*}

